Algorithm implementation and numerical analysis for the two-dimensional tempered fractional Laplacian

Tempered fractional Laplacian is the generator of the tempered isotropic L\'evy process [W.H. Deng, B.Y. Li, W.Y. Tian, and P.W. Zhang, Multiscale Model. Simul., 16(1), 125-149, 2018]. This paper provides the finite difference discretization for the two dimensional tempered fractional Laplacian $(\Delta+\lambda)^{\frac{\beta}{2}}$. Then we use it to solve the tempered fractional Poisson equation with Dirichlet boundary conditions and derive the error estimates. Numerical experiments verify the convergence rates and effectiveness of the schemes.

==> table/DC2x22y22g1a05.tex <==
\begin{table}[H]\fontsize{6.5pt}{10pt}\selectfont
  \centering
\begin{tabular}{ccccccccc}
\hline
$\beta \diagdown h$        &       & 1/2-1/4 & 1/4-1/8 & 1/8-1/16 & 1/16-1/32 & 1/32-1/64 & 1/64-1/128 & 1/128-1/256 \\\hline
      & $L_\infty$      & \multicolumn{1}{r}{8.960E-03} & 5.708E-03 & 2.149E-03 & 7.202E-04 & 2.307E-04 & 7.206E-05 & 2.214E-05 \\
0.2   &       & c.r.  & 0.6505  & 1.4092  & 1.5774  & 1.6426  & 1.6785  & 1.7027  \\\cline{3-9}
      & $L_2$      & \multicolumn{1}{r}{2.573E-03} & 2.073E-03 & 8.466E-04 & 2.966E-04 & 9.756E-05 & 3.101E-05 & 9.645E-06 \\
      &       & c.r.  & 0.3118  & 1.2917  & 1.5134  & 1.6040  & 1.6533  & 1.6851  \\\hline
      &$L_\infty$       & \multicolumn{1}{r}{2.761E-02} & 2.399E-02 & 1.081E-02 & 4.269E-03 & 1.608E-03 & 5.920E-04 & 2.151E-04 \\
0.5   &       & c.r.  & 0.2025  & 1.1499  & 1.3408  & 1.4087  & 1.4416  & 1.4608  \\\cline{3-9}
      &  $L_2$     & \multicolumn{1}{r}{7.981E-03} & 8.765E-03 & 4.306E-03 & 1.786E-03 & 6.932E-04 & 2.601E-04 & 9.569E-05 \\
      &       & c.r.  & -0.1353  & 1.0254  & 1.2699  & 1.3653  & 1.4140  & 1.4428  \\\hline
      &$L_\infty$       & \multicolumn{1}{r}{4.495E-02} & 6.132E-02 & 3.380E-02 & 1.603E-02 & 7.251E-03 & 3.219E-03 & 1.416E-03 \\
0.8   &       & c.r.  & -0.4481  & 0.8591  & 1.0766  & 1.1443  & 1.1717  & 1.1846  \\\cline{3-9}
      &$L_2$       & \multicolumn{1}{r}{1.499E-02} & 2.258E-02 & 1.359E-02 & 6.781E-03 & 3.164E-03 & 1.431E-03 & 6.366E-04 \\
      &       & c.r.  & -0.5907  & 0.7327  & 1.0028  & 1.0998  & 1.1448  & 1.1684  \\\hline
      &$L_\infty$       & \multicolumn{1}{r}{7.313E-02} & 1.470E-01 & 1.114E-01 & 6.907E-02 & 4.068E-02 & 2.358E-02 & 1.359E-02 \\
1.2   &       & c.r.  & -1.0069  & 0.3992  & 0.6900  & 0.7639  & 0.7869  & 0.7949  \\\cline{3-9}
      &$L_2$       & \multicolumn{1}{r}{4.250E-02} & 5.526E-02 & 4.531E-02 & 2.952E-02 & 1.791E-02 & 1.056E-02 & 6.144E-03 \\
      &       & c.r.  & -0.3789  & 0.2864  & 0.6179  & 0.7209  & 0.7623  & 0.7813  \\\hline
      &$L_\infty$       & \multicolumn{1}{r}{1.887E-01} & 1.950E-01 & 2.087E-01 & 1.619E-01 & 1.174E-01 & 8.362E-02 & 5.926E-02 \\
1.5   &       & c.r.  & -0.0477  & -0.0977  & 0.3662  & 0.4636  & 0.4894  & 0.4968  \\\cline{3-9}
      &$L_2$       & \multicolumn{1}{r}{1.306E-01} & 7.792E-02 & 8.588E-02 & 6.963E-02 & 5.190E-02 & 3.756E-02 & 2.684E-02 \\
      &       & c.r.  & 0.7455  & -0.1402  & 0.3026  & 0.4238  & 0.4668  & 0.4845  \\\hline
      &$L_\infty$       & \multicolumn{1}{r}{7.935E-01} & 1.327E-01 & 2.119E-01 & 2.265E-01 & 2.067E-01 & 1.821E-01 & 1.590E-01 \\
1.8   &       & c.r.  & 2.5801  & -0.6755  & -0.0959  & 0.1320  & 0.1828  & 0.1956  \\\cline{3-9}
      & $L_2$      & \multicolumn{1}{r}{3.730E-01} & 6.645E-02 & 9.175E-02 & 9.857E-02 & 9.179E-02 & 8.195E-02 & 7.210E-02 \\
      &       & c.r.  & 2.4888  & -0.4653  & -0.1035  & 0.1029  & 0.1636  & 0.1847  \\\hline
\end{tabular}%
\caption{The approximation of $(1-x^2)^2(1-y^2)^2$ with $\gamma=1+\frac{\alpha}{2}$}
\label{tab:DC2x22y22g1a05}%
\end{table}%


==> table/DC2x22y22g2_q.tex <==
\begin{table}[H]\fontsize{6.5pt}{10pt}\selectfont
  \centering
    \begin{tabular}{ccccccccc}
    \hline
$\beta \diagdown h$        &       & 1/2-1/4 & 1/4-1/8 & 1/8-1/16 & 1/16-1/32 & 1/32-1/64 & 1/64-1/128 & 1/128-1/256 \\\hline
      &$L_\infty$       & 6.052E-03 & 8.711E-04 & 1.662E-04 & 3.775E-05 & 9.163E-06 & 2.271E-06 & 5.664E-07 \\
0.2   &       & c.r.  & 2.7966  & 2.3901  & 2.1384  & 2.0425  & 2.0124  & 2.0036  \\\cline{3-9}
      &$L_2$       & 2.767E-03 & 3.595E-04 & 6.299E-05 & 1.421E-05 & 3.546E-06 & 9.033E-07 & 2.297E-07 \\
      &       & c.r.  & 2.9442  & 2.5128  & 2.1482  & 2.0027  & 1.9729  & 1.9752  \\\hline
      &$L_\infty$       & 2.625E-02 & 4.184E-03 & 8.062E-04 & 1.797E-04 & 4.298E-05 & 1.343E-05 & 4.392E-06 \\
0.5   &       & c.r.  & 2.6490  & 2.3758  & 2.1655  & 2.0637  & 1.6780  & 1.6129  \\\cline{3-9}
      &$L_2$       & 1.134E-02 & 1.634E-03 & 3.059E-04 & 7.326E-05 & 1.935E-05 & 5.188E-06 & 1.380E-06 \\
      &       & c.r.  & 2.7954  & 2.4172  & 2.0619  & 1.9207  & 1.8992  & 1.9100  \\\hline
      &$L_\infty$       & 6.941E-02 & 1.196E-02 & 2.298E-03 & 4.962E-04 & 1.564E-04 & 6.201E-05 & 2.442E-05 \\
0.8   &       & c.r.  & 2.5373  & 2.3797  & 2.2113  & 1.6653  & 1.3348  & 1.3443  \\\cline{3-9}
      &$L_2$       & 2.932E-02 & 4.665E-03 & 9.052E-04 & 2.217E-04 & 6.152E-05 & 1.772E-05 & 5.141E-06 \\
      &       & c.r.  & 2.6518  & 2.3658  & 2.0294  & 1.8496  & 1.7959  & 1.7851  \\\hline
      &$L_\infty$       & 1.969E-01 & 3.807E-02 & 7.477E-03 & 1.639E-03 & 7.344E-04 & 3.482E-04 & 1.760E-04 \\
1.2   &       & c.r.  & 2.3705  & 2.3480  & 2.1901  & 1.1578  & 1.0765  & 0.9841  \\\cline{3-9}
      &$L_2$       & 8.251E-02 & 1.520E-02 & 3.072E-03 & 7.428E-04 & 2.170E-04 & 7.197E-05 & 2.565E-05 \\
      &       & c.r.  & 2.4408  & 2.3064  & 2.0481  & 1.7751  & 1.5925  & 1.4884  \\\hline
      &$L_\infty$      & 3.914E-01 & 8.457E-02 & 1.764E-02 & 3.734E-03 & 1.826E-03 & 1.046E-03 & 6.580E-04 \\
1.5   &       & c.r.  & 2.2105  & 2.2614  & 2.2399  & 1.0325  & 0.8039  & 0.6682  \\\cline{3-9}
      &$L_2$       & 1.643E-01 & 3.451E-02 & 7.432E-03 & 1.756E-03 & 5.016E-04 & 1.813E-04 & 7.737E-05 \\
      &       & c.r.  & 2.2515  & 2.2152  & 2.0815  & 1.8076  & 1.4681  & 1.2287  \\\hline
      &$L_\infty$       & 7.395E-01 & 1.830E-01 & 4.250E-02 & 9.753E-03 & 3.143E-03 & 1.994E-03 & 1.501E-03 \\
1.8   &       & c.r.  & 2.0150  & 2.1059  & 2.1236  & 1.6337  & 0.6564  & 0.4100  \\\cline{3-9}
      &$L_2$       & 3.119E-01 & 7.624E-02 & 1.835E-02 & 4.442E-03 & 1.142E-03 & 3.620E-04 & 1.611E-04 \\
      &       & c.r.  & 2.0325  & 2.0551  & 2.0461  & 1.9594  & 1.6577  & 1.1680  \\\hline
\end{tabular}%
\caption{The approximation of $(1-x^2)^2(1-y^2)^2$ with $\gamma=2$}
\label{tab:DC2x22y22g2_q}%
\end{table}%


==> table/DC3x23y23g1a05.tex <==
\begin{table}[H]\fontsize{6.5pt}{10pt}\selectfont
  \centering
    \begin{tabular}{ccccccccc}
    \hline
$\beta \diagdown h$        &       & 1/2-1/4 & 1/4-1/8 & 1/8-1/16 & 1/16-1/32 & 1/32-1/64 & 1/64-1/128 & 1/128-1/256 \\\hline
      &$L_\infty$        & \multicolumn{1}{r}{4.569E-03} & 7.197E-03 & 2.995E-03 & 1.033E-03 & 3.348E-04 & 1.053E-04 & 3.253E-05 \\
0.2   &       & c.r.  & -0.6557  & 1.2647  & 1.5364  & 1.6249  & 1.6682  & 1.6955  \\\cline{3-9}
      &$L_2$       & \multicolumn{1}{r}{2.054E-03} & 2.071E-03 & 8.909E-04 & 3.113E-04 & 1.014E-04 & 3.200E-05 & 9.896E-06 \\
      &       & c.r.  & -0.0120  & 1.2171  & 1.5171  & 1.6176  & 1.6645  & 1.6931  \\\hline
      &$L_\infty$        & \multicolumn{1}{r}{1.277E-02} & 2.991E-02 & 1.521E-02 & 6.204E-03 & 2.367E-03 & 8.772E-04 & 3.199E-04 \\
0.5   &       & c.r.  & -1.2281  & 0.9757  & 1.2936  & 1.3901  & 1.4321  & 1.4551  \\\cline{3-9}
      &$L_2$       & \multicolumn{1}{r}{6.664E-03} & 8.536E-03 & 4.518E-03 & 1.875E-03 & 7.197E-04 & 2.675E-04 & 9.771E-05 \\
      &       & c.r.  & -0.3570  & 0.9179  & 1.2690  & 1.3811  & 1.4281  & 1.4529  \\\hline
      &$L_\infty$        & \multicolumn{1}{r}{2.907E-02} & 7.435E-02 & 4.770E-02 & 2.347E-02 & 1.076E-02 & 4.800E-03 & 2.117E-03 \\
0.8   &       & c.r.  & -1.3550  & 0.6403  & 1.0230  & 1.1260  & 1.1639  & 1.1809  \\\cline{3-9}
      &$L_2$       & \multicolumn{1}{r}{1.669E-02} & 2.101E-02 & 1.413E-02 & 7.102E-03 & 3.277E-03 & 1.467E-03 & 6.477E-04 \\
      &       & c.r.  & -0.3325  & 0.5728  & 0.9923  & 1.1156  & 1.1599  & 1.1791  \\\hline
      &$L_\infty$        & \multicolumn{1}{r}{2.434E-01} & 1.611E-01 & 1.560E-01 & 1.015E-01 & 6.059E-02 & 3.527E-02 & 2.036E-02 \\
1.2   &       & c.r.  & 0.5960  & 0.0456  & 0.6203  & 0.7444  & 0.7806  & 0.7927  \\\cline{3-9}
      &$L_2$       & \multicolumn{1}{r}{7.269E-02} & 4.548E-02 & 4.576E-02 & 3.068E-02 & 1.848E-02 & 1.079E-02 & 6.234E-03 \\
      &       & c.r.  & 0.6767  & -0.0089  & 0.5770  & 0.7311  & 0.7765  & 0.7913  \\\hline
      &$L_\infty$        & \multicolumn{1}{r}{7.882E-01} & 1.556E-01 & 2.842E-01 & 2.370E-01 & 1.749E-01 & 1.252E-01 & 8.883E-02 \\
1.5   &       & c.r.  & 2.3405  & -0.8689  & 0.2621  & 0.4384  & 0.4825  & 0.4948  \\\cline{3-9}
      &$L_2$       & \multicolumn{1}{r}{2.116E-01} & 5.861E-02 & 8.181E-02 & 7.129E-02 & 5.330E-02 & 3.829E-02 & 2.720E-02 \\
      &       & c.r.  & 1.8520  & -0.4813  & 0.1986  & 0.4195  & 0.4772  & 0.4933  \\\hline
      &$L_\infty$        & \multicolumn{1}{r}{2.130E+00} & 4.321E-01 & 2.443E-01 & 3.229E-01 & 3.062E-01 & 2.723E-01 & 2.383E-01 \\
1.8   &       & c.r.  & 2.3012  & 0.8228  & -0.4024  & 0.0764  & 0.1695  & 0.1922  \\\cline{3-9}
      &$L_2$       & \multicolumn{1}{r}{5.542E-01} & 1.748E-01 & 6.975E-02 & 9.511E-02 & 9.284E-02 & 8.319E-02 & 7.296E-02 \\
      &       & c.r.  & 1.6646  & 1.3255  & -0.4474  & 0.0349  & 0.1584  & 0.1893  \\\hline
\end{tabular}%
\caption{The approximation of $(1-x^2)^3(1-y^2)^3$ with $\gamma=1+\frac{\alpha}{2}$}
\label{tab:DC3x23y23g1a05}%
\end{table}%

==> table/DC3x23y23g2_q.tex <==
\begin{table}[H]\fontsize{6.5pt}{10pt}\selectfont
  \centering
\begin{tabular}{ccccccccc}
\hline
$\beta \diagdown h$        &       & 1/2-1/4 & 1/4-1/8 & 1/8-1/16 & 1/16-1/32 & 1/32-1/64 & 1/64-1/128 & 1/128-1/256 \\\hline
      &$L_\infty$       & 1.215E-02 & 1.543E-03 & 2.499E-04 & 5.212E-05 & 1.228E-05 & 3.015E-06 & 7.499E-07 \\
0.2   &       & c.r.  & 2.9768  & 2.6266  & 2.2613  & 2.0859  & 2.0257  & 2.0075  \\\cline{3-9}
      &$L_2$       & 3.131E-03 & 5.147E-04 & 7.998E-05 & 1.588E-05 & 3.679E-06 & 8.995E-07 & 2.234E-07 \\
      &       & c.r.  & 2.6050  & 2.6860  & 2.3326  & 2.1096  & 2.0322  & 2.0093  \\\hline
      &$L_\infty$       & 5.368E-02 & 8.185E-03 & 1.427E-03 & 2.980E-04 & 6.921E-05 & 1.683E-05 & 4.167E-06 \\
0.5   &       & c.r.  & 2.7132  & 2.5196  & 2.2599  & 2.1063  & 2.0397  & 2.0143  \\\cline{3-9}
      &$L_2$       & 1.376E-02 & 2.861E-03 & 4.931E-04 & 9.751E-05 & 2.201E-05 & 5.299E-06 & 1.307E-06 \\
      &       & c.r.  & 2.2659  & 2.5365  & 2.3384  & 2.1470  & 2.0548  & 2.0194  \\\hline
      &$L_\infty$       & 1.460E-01 & 2.542E-02 & 4.601E-03 & 9.412E-04 & 2.120E-04 & 5.044E-05 & 1.233E-05 \\
0.8   &       & c.r.  & 2.5223  & 2.4657  & 2.2895  & 2.1506  & 2.0713  & 2.0323  \\\cline{3-9}
      &$L_2$       & 3.745E-02 & 9.296E-03 & 1.724E-03 & 3.360E-04 & 7.289E-05 & 1.704E-05 & 4.139E-06 \\
      &       & c.r.  & 2.0104  & 2.4312  & 2.3588  & 2.2047  & 2.0967  & 2.0419  \\\hline
      &$L_\infty$       & 4.309E-01 & 8.869E-02 & 1.716E-02 & 3.470E-03 & 7.456E-04 & 1.687E-04 & 3.964E-05 \\
1.2   &       & c.r.  & 2.2805  & 2.3693  & 2.3063  & 2.2185  & 2.1437  & 2.0898  \\\cline{3-9}
      &$L_2$       & 1.108E-01 & 3.419E-02 & 7.147E-03 & 1.420E-03 & 2.939E-04 & 6.467E-05 & 1.500E-05 \\
      &       & c.r.  & 1.6965  & 2.2581  & 2.3310  & 2.2729  & 2.1842  & 2.1085  \\\hline
      &$L_\infty$       & 8.803E-01 & 2.077E-01 & 4.379E-02 & 9.182E-03 & 1.968E-03 & 4.333E-04 & 9.793E-05 \\
1.5   &       & c.r.  & 2.0836  & 2.2459  & 2.2536  & 2.2221  & 2.1831  & 2.1456  \\\cline{3-9}
      &$L_2$       & 2.268E-01 & 8.267E-02 & 1.954E-02 & 4.179E-03 & 8.818E-04 & 1.896E-04 & 4.212E-05 \\
      &       & c.r.  & 1.4562  & 2.0808  & 2.2251  & 2.2448  & 2.2174  & 2.1703  \\\hline
      &$L_\infty$       & 1.703E+00 & 4.670E-01 & 1.228E-01 & 2.931E-02 & 6.670E-03 & 1.527E-03 & 3.496E-04 \\
1.8   &       & c.r.  & 1.8664  & 1.9273  & 2.0667  & 2.1356  & 2.1269  & 2.1270  \\\cline{3-9}
      &$L_2$       & 4.393E-01 & 1.906E-01 & 5.239E-02 & 1.274E-02 & 2.971E-03 & 6.833E-04 & 1.568E-04 \\
      &       & c.r.  & 1.2049  & 1.8631  & 2.0401  & 2.1001  & 2.1203  & 2.1233  \\\hline
\end{tabular}%
\caption{The approximation of $(1-x)^3(1-y^2)^3$ with $\gamma=2$}
\label{tab:DC3x23y23g2_q}%
\end{table}%


==> table/soC2x22y22g2.tex <==
\begin{table}[H]\fontsize{6.5pt}{10pt}\selectfont
  \centering
\begin{tabular}{cccccccccc}
\hline
 $\beta \diagdown h$         &&    1/2   &    1/4   &    1/8   &    1/16  &    1/32  &    1/64  &    1/128 &    1/256\\ \hline
      &$L_\infty$       & 1.4024E-02 & 7.1083E-03 & 2.5650E-03 & 8.4428E-04 & 2.6753E-04 & 8.2960E-05 & 2.5349E-05 & 7.6603E-06 \\
0.2   &       & c.r.  & 0.9803  & 1.4706  & 1.6032  & 1.6580  & 1.6892  & 1.7105  & 1.7264  \\\cline{3-10}
      &$L_2$       & 8.6666E-03 & 5.0419E-03 & 1.9281E-03 & 6.5640E-04 & 2.1240E-04 & 6.6772E-05 & 2.0593E-05 & 6.2641E-06 \\
      &       & c.r.  & 0.7815  & 1.3868  & 1.5546  & 1.6278  & 1.6695  & 1.6971  & 1.7170  \\\hline
      &$L_\infty$       & 3.7803E-02 & 2.3665E-02 & 1.0158E-02 & 3.9349E-03 & 1.4657E-03 & 5.3567E-04 & 1.9365E-04 & 6.9522E-05 \\
0.5   &       & c.r.  & 0.6758  & 1.2202  & 1.3682  & 1.4247  & 1.4522  & 1.4679  & 1.4779  \\\cline{3-10}
      &$L_2$       & 2.4384E-02 & 1.6796E-02 & 7.4130E-03 & 2.9212E-03 & 1.1009E-03 & 4.0553E-04 & 1.4735E-04 & 5.3072E-05 \\
      &       & c.r.  & 0.5378  & 1.1800  & 1.3435  & 1.4078  & 1.4409  & 1.4606  & 1.4732  \\\hline
      &$L_\infty$       & 6.4025E-02 & 5.0133E-02 & 2.6110E-02 & 1.2198E-02 & 5.4804E-03 & 2.4227E-03 & 1.0630E-03 & 4.6469E-04 \\
0.8   &       & c.r.  & 0.3529  & 0.9412  & 1.0980  & 1.1543  & 1.1777  & 1.1885  & 1.1938  \\\cline{3-10}
      &$L_2$       & 4.2724E-02 & 3.6399E-02 & 1.9157E-02 & 8.9819E-03 & 4.0460E-03 & 1.7920E-03 & 7.8730E-04 & 3.4443E-04 \\
      &       & c.r.  & 0.2311  & 0.9260  & 1.0928  & 1.1505  & 1.1749  & 1.1866  & 1.1927  \\\hline
      &$L_\infty$       & 9.9029E-02 & 1.0612E-01 & 7.2876E-02 & 4.4876E-02 & 2.6588E-02 & 1.5503E-02 & 8.9735E-03 & 5.1752E-03 \\
1.2   &       & c.r.  & -0.0997  & 0.5422  & 0.6995  & 0.7552  & 0.7782  & 0.7888  & 0.7940  \\\cline{3-10}
      &$L_2$       & 6.7803E-02 & 8.0164E-02 & 5.5491E-02 & 3.4120E-02 & 2.0173E-02 & 1.1745E-02 & 6.7921E-03 & 3.9151E-03 \\
      &       & c.r.  & -0.2416  & 0.5307  & 0.7016  & 0.7582  & 0.7804  & 0.7901  & 0.7948  \\\hline
      &$L_\infty$       & 1.2076E-01 & 1.6509E-01 & 1.3927E-01 & 1.0611E-01 & 7.8128E-02 & 5.6668E-02 & 4.0767E-02 & 2.9176E-02 \\
1.5   &       & c.r.  & -0.4511  & 0.2454  & 0.3923  & 0.4417  & 0.4633  & 0.4751  & 0.4826  \\\cline{3-10}
      &$L_2$       & 8.2856E-02 & 1.2783E-01 & 1.0921E-01 & 8.3270E-02 & 6.1236E-02 & 4.4359E-02 & 3.1880E-02 & 2.2799E-02 \\
      &       & c.r.  & -0.6256  & 0.2272  & 0.3912  & 0.4434  & 0.4651  & 0.4766  & 0.4837  \\\hline
      &$L_\infty$       & 1.3327E-01 & 2.3545E-01 & 2.3908E-01 & 2.2130E-01 & 1.9986E-01 & 1.7896E-01 & 1.5956E-01 & 1.4185E-01 \\
1.8   &       & c.r.  & -0.8211  & -0.0221  & 0.1115  & 0.1470  & 0.1594  & 0.1655  & 0.1697  \\\cline{3-10}
      &$L_2$       & 8.9855E-02 & 1.8540E-01 & 1.9152E-01 & 1.7788E-01 & 1.6072E-01 & 1.4390E-01 & 1.2827E-01 & 1.1400E-01 \\
      &       & c.r.  & -1.0450  & -0.0468  & 0.1066  & 0.1463  & 0.1595  & 0.1659  & 0.1701  \\\hline
\end{tabular}%
\caption{The error of $(1-x^2)^2(1-y^2)^2$ with $\gamma=1+\frac{\beta}{2}$}
\label{tab:soC2x22y22g2}
\end{table}%


==> table/soC3x23y23g2.tex <==
\begin{table}[H]\fontsize{6.5pt}{10pt}\selectfont
  \centering
    \begin{tabular}{cccccccccc}
    \hline
$\beta \diagdown h$         &&    1/2   &    1/4   &    1/8   &    1/16  &    1/32  &    1/64  &    1/128 &    1/256\\ \hline
         &$L_\infty$ & 1.092E-02 & 1.429E-03 & 2.456E-04 & 5.303E-05 & 1.265E-05 & 3.120E-06 & 7.769E-07 & 1.940E-07 \\
0.2      && c.r.  & 2.9335  & 2.5409  & 2.2112  & 2.0673  & 2.0199  & 2.0058  & 2.0019  \\\cline{3-10}
         &$L_2$& 5.709E-03 & 9.098E-04 & 1.519E-04 & 3.191E-05 & 7.553E-06 & 1.858E-06 & 4.624E-07 & 1.154E-07 \\
         && c.r.  & 2.6497  & 2.5823  & 2.2511  & 2.0790  & 2.0230  & 2.0067  & 2.0022 \\\hline
         &$L_\infty$& 3.401E-02 & 5.026E-03 & 9.103E-04 & 1.964E-04 & 4.635E-05 & 1.135E-05 & 2.816E-06 & 7.018E-07\\
0.5      && c.r.  & 2.7584  & 2.4651  & 2.2128  & 2.0829  & 2.0302  & 2.0109  & 2.0043  \\\cline{3-10}
         &$L_2$& 1.779E-02 & 3.198E-03 & 5.743E-04 & 1.202E-04 & 2.795E-05 & 6.803E-06 & 1.684E-06 & 4.196E-07 \\
         && c.r.  & 2.4757  & 2.4771  & 2.2562  & 2.1046  & 2.0387  & 2.0140  & 2.0050\\\hline
         &$L_\infty$& 6.517E-02 & 1.021E-02 & 1.869E-03 & 3.936E-04 & 9.056E-05 & 2.180E-05 & 5.359E-06 & 1.330E-06\\
0.9      && c.r.  & 2.6745  & 2.4497  & 2.2471  & 2.1198  & 2.0545  & 2.0242  & 2.0111  \\\cline{3-10}
         &$L_2$& 3.424E-02 & 6.479E-03 & 1.203E-03 & 2.472E-04 & 5.577E-05 & 1.328E-05 & 3.250E-06 & 8.045E-07 \\
         && c.r.  & 2.4017  & 2.4294  & 2.2827  & 2.1481  & 2.0697  & 2.0314  & 2.0140\\\hline
         &$L_\infty$& 1.227E-01 & 2.041E-02 & 3.816E-03 & 7.810E-04 & 1.714E-04 & 3.949E-05 & 9.397E-06 & 2.281E-06\\
1.2      && c.r.  & 2.5875  & 2.4193  & 2.2887  & 2.1883  & 2.1175  & 2.0712  & 2.0427  \\\cline{3-10}
         &$L_2$& 6.524E-02 & 1.279E-02 & 2.486E-03 & 5.057E-04 & 1.090E-04 & 2.474E-05 & 5.822E-06 & 1.404E-06 \\
         && c.r.  & 2.3505  & 2.3632  & 2.2977  & 2.2133  & 2.1401  & 2.0870  & 2.0523 \\\hline
         &$L_\infty$& 1.832E-01 & 3.221E-02 & 6.326E-03 & 1.314E-03 & 2.840E-04 & 6.332E-05 & 1.449E-05 & 3.388E-06 \\
1.5      && c.r.  & 2.5081  & 2.3483  & 2.2670  & 2.2105  & 2.1649  & 2.1273  & 2.0968  \\\cline{3-10}
         &$L_2$& 9.879E-02 & 1.984E-02 & 4.073E-03 & 8.542E-04 & 1.837E-04 & 4.056E-05 & 9.189E-06 & 2.129E-06 \\
         && c.r.  & 2.3158  & 2.2842  & 2.2536  & 2.2174  & 2.1790  & 2.1422  & 2.1097  \\\hline
         &$L_\infty$& 2.670E-01 & 5.039E-02 & 1.084E-02 & 2.435E-03 & 5.555E-04 & 1.277E-04 & 2.955E-05 & 6.874E-06 \\
1.8      && c.r.  & 2.4057  & 2.2161  & 2.1546  & 2.1323  & 2.1206  & 2.1119  & 2.1041  \\\cline{3-10}
         &$L_2$& 1.465E-01 & 3.041E-02 & 6.769E-03 & 1.538E-03 & 3.520E-04 & 8.098E-05 & 1.871E-05 & 4.345E-06 \\
         && c.r.  & 2.2681  & 2.1675  & 2.1382  & 2.1270  & 2.1200  & 2.1135  & 2.1068  \\\hline
    \end{tabular}%
    \caption{The error of $(1-x^2)^3(1-y^2)^3$ with $\gamma=2$}
  \label{tab:soC3x23y23g2}%
\end{table}%


